Formally Verified C Code Generation from Hybrid Communicating Sequential Processes

Hybrid Communicating Sequential Processes (HCSP) is a formal model for hybrid systems, including primitives for evolution along an ordinary differential equation (ODE), communication, and parallel composition. Code generation is needed to convert HCSP models into code that can be executed in practice, and the correctness of this conversion is essential to ensure that the generated code accurately reflects the formal model. In this paper, we propose a code generation algorithm from HCSP to C with POSIX library for concurrency. The main difficulties include how to bridge the gap between the synchronized communication model in HCSP and the use of mutexes for synchronization in C, and how to discretize evolution along ODEs and support interrupt of ODE evolution by communication. To prove the correctness of code generation, we define a formal semantics for POSIX C, and build transition system models for both HCSP and C programs. We then define an approximate bisimulation relation between traces of transition systems, and show that under certain robustness conditions for HCSP, the generated C program is approximately bisimilar to the original model. Finally, we evaluate the code generation algorithm on a detailed model for automatic cruise control, showing its utility on real-world examples.

==> commentaux.tex <==
\newcommand{\Var}{\mathcal{V}}
\newcommand{\Chan}{\mathcal{C}}

\newcommand{\wsl}[1]{{\color{red} #1}}
\newcommand{\creturn}[1]{\textbf{return}\ #1}
\newcommand{\ereturn}{\textbf{retv}}
\newcommand{\vreturn}{\textbf{ret}}
\newcommand{\hP}{h^{\prime}}
\newcommand{\PHI}{\mathbf{\Phi}}

% Constructors of HCSP
\newcommand{\pskip}{\textmd{skip}}
\newcommand{\pstop}{\varepsilon}
\newcommand{\evofun}[2]{\mathcal{#1}(\dot{#2},#2)=0}
\newcommand{\evolution}[3]{\langle \mathcal{#1}(\dot{#2},#2)=0 \& #3\rangle}
\newcommand{\evo}[3]{\langle \dot{#1}=#2\& #3\rangle}
\newcommand{\evon}[2]{\langle \dot{#1}=#2\rangle}
\newcommand{\imitate}[4]{\langle \mathcal{#1}(\dot{#2},#2)=0; #3 \& #4\rangle}
\newcommand{\pwait}{\textrm{wait}}
\newcommand{\seman}[1]{[\![#1]\!]}
\newcommand{\returnv}{\textbf{ret}}
\newcommand{\mainthread}{\textbf{t}_m}

\newcommand{\exempt}[4]{#1 \unrhd \talloblong_{#2} (#3 \rightarrow #4)}
\newcommand{\exemptS}[3]{#1 \unrhd (#2 \rightarrow #3)}
\newcommand{\external}[3]{\talloblong_{#1} (#2 \rightarrow #3)}
\newcommand{\internal}[3]{\sqcup_{#1} (#2 \rightarrow #3)}
\newcommand{\lr}{\talloblong}
\newcommand{\fracN}[2]{\frac{\textstyle #1}{\textstyle #2}}
\newcommand{\almost}[1]{\lceil #1 \rceil}
\newcommand{\specF}[4]{\{#2\} #1 \{#3; \; #4\}}
\newcommand{\chop}{\smallfrown}
\newcommand{\close}{\textit{cl}}
\newcommand{\chanset}{\textit{chans}}
 
\newcommand{\pdef}{\ \widehat{=}\ } 
\newcommand{\angles}[1]{\langle #1 \rangle}
\newcommand{\prepeat}[1]{#1^*} 
\newcommand{\oomit}[1]{}
\newcommand{\IFE}[3]{\textbf{if}\ #1\ #2\ \textbf{else}\ #3}
\newcommand{\IFT}[2]{\textrm{if}\ #1\ \textrm{then}\ #2}
\newcommand{\for}[4]{\textbf{for}(#1, #2, #3)\ #4}
\newcommand{\compat}{\operatorname{compat}}
\newcommand{\rdy}{\mathit{rdy}}
 
%defined for C language
\newcommand{\cwhile}[2]{\textbf{while}\ #1 \ #2}
\newcommand{\clock}[2]{\textbf{lock}\ #1\ #2}
\newcommand{\cunlock}[2]{\textbf{unlock}\ #1\ #2}
\newcommand{\cwait}[3]{\textbf{cwait}\ #1\ #2\ #3}
\newcommand{\lock}[1]{\textbf{lock}\ #1}
\newcommand{\unlock}[1]{\textbf{unlock}\ #1}
\newcommand{\wait}[2]{\textbf{cwait}\ #1\ #2}
\newcommand{\cwaitp}[3]{\textbf{cwait'}\ #1\ #2}
\newcommand{\csignal}[2]{\textbf{signal}\ #1 \ #2}
\newcommand{\signal}[1]{\textbf{signal}\ #1}
\newcommand{\create}[3]{\textbf{create}\ #1\ #2\ #3}
\newcommand{\join}[1]{\textbf{join}\ #1}

\newcommand{\elock}{\textit{lock}}
\newcommand{\eunlock}{\textit{unlock}}
\newcommand{\ewait}{\textit{wait}}
\newcommand{\esignal}{\textit{sig}}
\newcommand{\toc}{\textit{HtoC}}
\newcommand{\DHCSP}{\textit{HtoD}}
 


\newcommand{\comment}[1]{{\color{blue} #1}}


\newcommand{\sm}[1]{$#1$}

\newcommand{\qq}{q}
\newcommand{\labeld}{\textit{dis}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\ff}{\mathbf{f}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\euler}{\xi}
\newcommand{\nstop}{\textbf{stop}}


==> proof.tex <==
\oomit{We prove the result by induction on the transitions of HCSP. We classify the proof into three cases:
\begin{itemize}
    \item[(1)] $l=\tau$, corresponding to the execution of  $\pskip$, $x:=e$, and evaluation of conditions in if-else, while, continuous evolution and interrupt.

    \item[(2)] $l=\langle ch, v\rangle$, corresponding to the occurrence of a synchronised communication.
    

    \item[(3)] $l = \langle d, \rdy\rangle$, corresponding to the execution of ODEs, communication interrupts, and communications (for waiting cases). 
\end{itemize}
}

\subsection{Proof of discrete bisimulation}
\label{sec:proof-discrete-bisimulation}

In this section, we sketch the proof of exact bisimulation  between discretized HCSP and generated C code. The overall strategy is to define a bisimulation relation between the states of HCSP and concurrent C, and show that transitions on the HCSP side and C side correspond under this relation.

First, we note that there is only one mutex to protect all shared resources in the generated C code. The translation of $\mathsf{wait\_comm}$ (and hence its special cases $\mathsf{delay}$, $\mathsf{input}$ and $\mathsf{output}$) all lock the mutex at the beginning and unlock it at the end. Hence, we can consider its execution to consist of a small number of atomic blocks. The execution of $\mathsf{wait\_comm}$ may be blocked in the middle for two different reasons:
\begin{enumerate}
\item[a)] After setting the channel sides, at least one communication is ready to be performed. After nondeterministically choosing a communication to perform and reserve it by setting the thread state on the other side, it signals the other side and waits for it to respond. The thread returns from blocking when the other side responds with a signal.

\item[b)] After setting the channel sides, no communication is ready to be performed. Then it enters into waiting mode for both communications and a time limit. The thread returns from blocking when either the time limit is reached, or one of the matching communications is ready.
\end{enumerate}
The translation of $\mathsf{delay}$, $\mathsf{input}$ and $\mathsf{output}$ are simply special cases of the above. For $\mathsf{delay}$ it does not attempt to seek a matching communication. For $\mathsf{input}$/$\mathsf{output}$, the time limit for waiting is $\infty$. We use subscript $\mathsf{a}$ and $\mathsf{b}$ to denote the second atomic block of execution in the cases a) and b), respectively.

Hence, each execution of $\mathsf{wait\_comm}$ consists of two atomic blocks. The execution of each matching communication then consist of four atomic blocks (two on the input side and two on the output side), one of which updates the value of the variable to be read on the input side. There are two cases, depending on whether the input side or the output side is ready first. The first case, when the input is ready first, is illustrated as follows.
\begin{center}
\includegraphics[scale=0.20]{images/input_first2.png}
\end{center}
The transition $ch.e$ on the HCSP side corresponds to four atomic steps on the C side. In step 1, the input side is ready and blocks on waiting for the output side. In step 2, the output side starts and detects the input is ready, copies the value to be sent into the channel, reserves the communication and signals the input side. In step 3, the input side copies the value in the channel into the variable to be read, cleans up after the communication, and finally signals back to the output side. In step 4, the output side cleans up the communication as well upon receiving the signal. In this sequence, the value to be read is updated on the third step. Hence, the proof strategy is as follows: the bisimulation relation is defined so that the HCSP program $ch?x~\|~ch!e$ is related to the first three states on the C side, while $\mathsf{skip}~\|~\mathsf{skip}$ is related to the final two states (as indicated by the dashed arrows).

\oomit{The case when the output is ready first is illustrated as follows. This is mostly symmetric to the above.
 The main differences are that the value to be communicated is copied into the channel in step 1, and read in step 2.
\begin{center}
\includegraphics[scale=0.16]{images/output_first2.png}
\end{center}}
 %Hence, we define the bisimulation relation so that the HCSP program $ch?x~\|~ch!e$ is related to the first two states on the C side, while $\mathsf{skip}~\|~\mathsf{skip}$ is related to the final three states.

The case when the output is ready first is mostly symmetric to the above.
We next consider the case of bisimulation relation for delays. The transition $\langle d,\rdy\rangle$ advances the clock on the HCSP side, and should correspond to updating the global variable $\texttt{currentTime}$ on the C side. This may correspond to multiple atomic steps on the C side, as illustrated below.
\begin{center}
\includegraphics[scale=0.21]{images/delay.png}
\end{center}
In step 1, only the first thread is delayed by 10, incrementing $\texttt{localTime}$ of that thread by 10 but leaving the global $\texttt{currentTime}$ unchanged. In step 2, the second thread is delayed by 10, leading to the increment of $\texttt{currentTime}$ as well. Hence, the bisimulation relation should be defined so that the HCSP program $\mathsf{wait}(10)~\|~\mathsf{wait}(10)$ is related to the first two states on the C side, while $\mathsf{skip}~\|~\mathsf{skip}$ is related to the final state.

In summary, the overall strategy of the bisimulation proof is as follows:
(1) Bisimulation relation is defined between the states on the HCSP side and C side. There is a direct correspondence between processes in HCSP and threads in C. For each process/thread, if the HCSP program and C program that remains to be executed agree, then the other parts of the C state have their default values: thread state is $\texttt{RUNNING}$ and $\texttt{localTime}$ should agree with $\texttt{currentTime}$. There are several other cases where the program to be executed on the C side runs ahead or behind the HCSP program, which is indicated by different conditions on the other parts of the C state.
(2) For each atomic block of execution in $\mathsf{wait\_comm}$,
%(and hence its special cases $\mathsf{delay}$, $\mathsf{input}$ and $\mathsf{output}$), 
we prove that if the starting state satisfies the bisimulation relation, then the ending state satisfies it as well. There are several cases to consider, depending on whether the C program to be executed runs ahead, behind, or agrees with the HCSP program. We also make use of the fact that in certain states, some threads in C are blocked by the condition variable.


==> sec_case_study.tex <==
\section{Case Study}\label{CaseStudy}

We adopt the realistically-scaled Automatic Cruise Control System (ACCS for short) from~\cite{DBLP:journals/tcs/XuWZJTZ22} as the case study. \comment{The HCSP model of ACCS is moderately large and covers all the concerned features of HCSP 
and it is robustly safe (Sect.~\ref{sec:robustly-safe}) and hence can be discretized using our approach.}
In this section, we translate this HCSP model to the C code and compare its execution with the simulation of the HCSP model~\cite{DBLP:journals/tcs/XuWZJTZ22} and the execution of the C code generated directly from the original $\textsc{AADL}\oplus\textsc{S/S}$ model~\cite{DBLP:conf/utp/ZhanLWTXZ19}.

\oomit{
\begin{figure*}
\centering
\includegraphics[scale=0.45]{CCS.pdf}
\caption{Automatic Cruise Control System (borrowed from~\cite{DBLP:journals/tcs/XuWZJTZ22})}
\label{fig:CCS}
\end{figure*}
}

\subsection{The Automatic Cruise Control System}\label{ACCS_arch}

The architecture of ACCS consists of three layers. The physical layer is the physical vehicle. The software level defines control of the system and it contains three processes for obstacle detection, velocity control, and panel control, and each process is composed of several threads. These processes interact with the environment (the physical layer) through devices. The platform layer consists of a bus and a processor. The connections between processes and devices could be bound to the bus and all the threads are bound to the processor, with HPF (High-Priority-First) scheduling policy.

% The execution of ACCS is as follows. A vehicle is placed at the starting point initially and the driver can accelerate (\texttt{inc}) and decelerate (\texttt{dec}) the vehicle by the \texttt{user\_panel}. Thread \texttt{pan\_ctr\_th} deals with the commands from the driver and then sends desired velocities (\texttt{des\_v}) to the discrete PI controller (thread \texttt{PI\_ctr}). Meanwhile, process \texttt{obs\_det} detects the obstacles ahead by a \texttt{camera} and a \texttt{radar} and provides the velocity controller process (\texttt{vel\_ctr}) with the real-time position of obstacle (\texttt{obs\_pos}). Thread \texttt{velo\_voter} in process \texttt{vel\_ctr} monitors the velocity of the vehicle using \texttt{laser} and another device located on one \texttt{wheel} of the vehicle and produces the real-time velocity of the vehicle (\texttt{veh\_v}) to the discrete PI controller \texttt{PI\_ctr} and the emergency control thread (\texttt{emerg}). Based on the real-time velocity of vehicle and the desired velocity received, \texttt{PI\_ctr} computes a desired acceleration (\texttt{des\_a}) which will be sent to \texttt{emerg}. Finally, \texttt{emerg} collects the real-time position (\texttt{veh\_pos} by \texttt{GPS}) and velocity of the vehicle, the desired velocity set by the driver, and the real-time position of the obstacle to work out a \texttt{command}, by some emergency control strategy, which will update the acceleration of the vehicle through \texttt{actuator}. The vehicle moves according to the new acceleration and the above procedure repeats. 

\subsection{Translation from HCSP to C}

In work~\cite{DBLP:conf/utp/ZhanLWTXZ19}, combined models of $\textsf{AADL}\oplus\textsf{S/S}$ are translated to C code directly. \oomit{The translation is done by the following steps: (1) the AADL part is translated to C following the execution semantics of AADL; (2) the Simulink/Stateflow part is translated using the existing C code generation facility in Matlab; (3) the architecture part is implemented by a library in C that includes thread scheduling protocols and so on; and (4) the combined model is translated by integrating the C codes generated from the above three parts. However, the interaction (communication) between components is implemented by shared variables (without \textsf{pthreads}) and the correctness of the translation has not been proved.
}
In this paper, 
%we generate the C code of ACCS from its HCSP model obtained from~\cite{DBLP:journals/tcs/XuWZJTZ22}. The HCSP model is specified by a formal language and therefore verifiable. Thus, the C code generated from HCSP models is more reliable than~\cite{DBLP:conf/utp/ZhanLWTXZ19}.
we generate the C code of the case study from its HCSP model which has been verified in~\cite{DBLP:journals/tcs/XuWZJTZ22}. Since the correctness of the translation is guaranteed (Sect.~\ref{sec:correct}), the generated code, especially the code for the controller (the velocity control mentioned in Sect.~\ref{ACCS_arch}), satisfies the safety requirement and therefore is reliable.
We use $\mathsf{pthreads}$ to implement the communication between processes and the correctness of the code generation has been proved in Sect.~\ref{sec:correct}. The generated C code is of 3500--4000 lines, longer than the C code (about 2500 lines) generated by \cite{DBLP:conf/utp/ZhanLWTXZ19}. 
%In spite of its reliability and correctness, the generated code is, however, verbose: 3500--4000 lines of C code (while about 2500 lines by the translation of work \cite{DBLP:conf/utp/ZhanLWTXZ19}). 
One major reason is that the generated C code in this paper is approximately bisimilar to the original $\textsf{AADL}\oplus\textsf{S/S}$ model of ACCS, which means the detailed behaviours of ACCS are reflected in the C code and vice versa, while it is not the case for~\cite{DBLP:conf/utp/ZhanLWTXZ19} where no such bisimulation can be guaranteed. 
%In addition, the generated C code of this paper is more readable than~\cite{DBLP:conf/utp/ZhanLWTXZ19}, because in the latter, the C code of the Simulink part of ACCS is generated by the tool in Matlab, which introduces 

\subsection{Comparison}

We consider the following scenario. At the beginning, the driver pushes the \texttt{inc} button three times with time interval $0.5$s in between to set a desired speed to $3$m/s. After $30$s, the driver pushes the \texttt{dec} button twice in $0.5$s time intervals to decrease the desired speed. On the obstacle side, we assume that the obstacle appears at time $10$s and position $35$m, then moves ahead with velocity $2$m/s, before finally moving away at time $20$s and position $55$m. 

\oomit{
We adopt the parameters setting of Table 1 in~\cite{DBLP:journals/tcs/XuWZJTZ22} for the threads and devices in the ACCS of Fig.~\ref{fig:CCS}, except that the deadline of thread \texttt{pan\_ctr\_th} is shrunk to $50$ms in this paper.
We compare our results with the work~\cite{DBLP:conf/utp/ZhanLWTXZ19} and the simulation of the HCSP model of ACCS~\cite{DBLP:journals/tcs/XuWZJTZ22}. It should be noted that bus latency is not considered in~\cite{DBLP:conf/utp/ZhanLWTXZ19}. Thus, to make it fair, we only consider the case with on bus latency, i.e., we ignore the \texttt{bus} component in Fig.~\ref{fig:CCS}. Actually, \texttt{bus} has no impact on the study, as we only concern the translation from HCSP to C in this paper and each \texttt{bus} in the original $\textsf{AADL}\oplus\textsf{S/S}$ model will be translated to a specific process in the obtained HCSP model by~\cite{DBLP:journals/tcs/XuWZJTZ22}.
}

The top of Fig.~\ref{fig:veh_v_s} shows the execution results of the vehicle speed, where the black line denotes the desired velocity set by the driver, and the red, green, and blue lines denote the results of our work, the work of~\cite{DBLP:conf/utp/ZhanLWTXZ19}, and the simulation of the HCSP model of ACCS~\cite{DBLP:journals/tcs/XuWZJTZ22}, respectively. We can see that the execution result (red line) of the generated C code is almost the same with the simulation (blue line) of its HCSP model.
\comment{Specifically, the average relative error (ARE) between the time series of the velocity generated from the HCSP model and its C code is $0.138\%$ with the variance $4.686\times10^{-5}$.}
Besides, we can also observe that there is negligible difference between the results  of the C code generated by~\cite{DBLP:conf/utp/ZhanLWTXZ19} (green line) and the C code generated in this paper (red line):
\comment{the ARE is $0.182\%$ with the variance $4.232\times10^{-3}$.}
Readers can refer to~\cite{DBLP:journals/tcs/XuWZJTZ22} for more details about this example.


\comment{It should be noted that although the generated C code in this paper is longer and somewhat less efficient than the C code generated directly from the original graphical model~\cite{DBLP:conf/utp/ZhanLWTXZ19}, the former is more reliable because it is translated from the (formal) HCSP model, which can be verified by tools like HHLPy~\cite{DBLP:conf/fm/ShengBZ23}, and moreover, the correctness of the translation can be guaranteed (Sect.~\ref{sec:correct}).}
%These results are quite similar, though some negligible latency, largely due to our discretization of the ODEs, can be observed in the result of our work (red line). 

\oomit{
From all these results, we can see that the vehicle accelerates to the desired speed ($3$m/s) in $10$s. The fluctuation during $[2\text{s},10\text{s}]$ reflects feature of PI controllers.
%: the vehicle under control rushes over the desired velocity and then returns about desired velocity soon. 
It then decelerates to avoid the collision onto the obstacle ahead. After the obstacle moves away (at $20$s), the vehicle accelerates again to the desired speed. At $30$s, the driver pushes the \texttt{dec} button to adjust the desired velocity to $1$m/s and we can see that the vehicle decelerates to $1$m/s in about $6$s under the PI controller. The positions of the vehicle and of the obstacle with respect to time are shown at the bottom of Fig.~\ref{fig:veh_v_s}.
%\vspace{-3mm}
}

\begin{figure}[h]
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{nobus_v.pdf}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{nobus_s.pdf}
\end{minipage}
\caption{Comparison of execution results}
\label{fig:veh_v_s}
\end{figure}
